The Economics and Econometrics of Gene-Environment Interplay

Economists and social scientists have debated the relative importance of nature (one's genes) and nurture (one's environment) for decades, if not centuries. This debate can now be informed by the ready availability of genetic data in a growing number of social science datasets. This paper explores the potential uses of genetic data in economics, with a focus on estimating the interplay between nature (genes) and nurture (environment). We discuss how economists can benefit from incorporating genetic data into their analyses even when they do not have a direct interest in estimating genetic effects. We argue that gene--environment (GxE) studies can be instrumental for (i) testing economic theory, (ii) uncovering economic or behavioral mechanisms, and (iii) analyzing treatment effect heterogeneity, thereby improving the understanding of how (policy) interventions affect population subgroups. We introduce the reader to essential genetic terminology, develop a conceptual economic model to interpret gene-environment interplay, and provide practical guidance to empirical researchers.

==> OldSection2.tex <==


In practice, measures of children’s endowments (e.g., birth weight) are rarely clean of parental investments, and parental investments are serially correlated over time, posing a formidable empirical challenge to accurately identify dynamic complementarities in skill formation. Genetic data has the major advantage that it is fixed at conception and invariant over the life cycle, and therefore insensitive to (parental) behavior.

Finally, although there has been a heated debate about the policy-relevance of heritability studies \citep{Goldberger1979,taubman1981heritability,Manski2011}, the study of $G \times E$ interplay can contribute novel evidence for policy makers. For example, it may become possible to identify environments or policies that reduce or even neutralize genetic inequalities, or that help individuals better reach their genetic potential \citep{Bierut2018}. Although the current predictive power of genetic indices precludes \textit{individual} prediction of future traits such as disease outcomes, it performs well at the \textit{group}- or \textit{population}-level. Understanding how environmental exposures affect social or economic outcomes for different genetically at risk groups may be useful to policy makers. For example, genetic information could then be used preventatively by informing individuals (e.g., by a medical doctor) to avoid environments that may harm them. The validity of such policy recommendations stemming from empirical studies crucially hinges on the correct specification and interpretation of empirical models. In this study, we provide a guide to empirical researchers, discussing this in detail.




\textit{Why is now the time to realize our goals?}
Recent technological advances in the mapping of the genome, rapid reductions in the costs of measuring genetic variation across people, and fast growth in sample sizes have led to substantial growth in the power of genetic discovery studies, also known as genome-wide association studies (GWAS).\footnote{See \hyperref[sec:G]{Section~\ref*{sec:G}} for a detailed discussion of GWAS and \hyperref[sec:glossary]{Appendix~\ref*{sec:glossary}} for a glossary.} Economists have been pioneers in pushing the GWAS approach to uncover the genetic underpinnings of a range of social and economic outcomes, such as educational attainment \citep{Rietveld2013,Okbay2016,lee2018gene}, subjective well-being \citep{Okbay2016well}, and risk aversion \citep{KarlssonLinner2019}. These GWAS discovery studies have enabled researchers to construct highly predictive polygenic indices (PGIs) that summarize the effects of multiple genetics variants. For example, the PGI for educational attainment, constructed on the basis of the latest GWAS, has a predictive power ($R^2$) of $\sim$12\% in an independent hold-out sample, making its effects detectable with 80\% power at a $p$-value threshold of 0.05 in a sample of only 70 individuals \citep{lee2018gene}.\footnote{This is a substantial improvement over the use of individual SNPs. For example, the SNP most strongly associated with educational attainment has an $R^2$ of only $\sim$0.02\% %, equivalent to approximately 1 month of schooling per ``allele''
\citep{Rietveld2013,Okbay2016}.} Today, results of GWASs are available for hundreds of human traits (see e.g., https://atlas.ctglab.nl/) making it possible to study $G \times E$ interplay in these traits, even in studies of relatively small size by using the power of polygenic indices.

Polygenic indices are now available or can be constructed in several datasets commonly used by economists.\footnote{Examples of such datasets include the Avon Longitudinal Study of Parents and Children (ALSPAC), the German Socioeconomic Panel (GSOEP), the National Longitudinal Study of Adolescent to Adult Health (AddHealth), the English Longitudinal Study of Ageing (ELSA), the Framingham Heart Study (FHS), the Health and Retirement Study (HRS), the Millenium Cohort Study (MCS), the National Child Development Study (NCDS), the National Survey of Health and Development Cohort (NSHD), the UK Household Longitudinal Study (UKHLS, `Understanding Society'), the UK Biobank (UKB), and the Wisconsin Longitudinal Study (WLS).} Until recently, accessing and processing the genetic data in these surveys required specific software and skills. With the progress in polygenic prediction, and the efforts of, e.g., the Health and Retirement Study and the SSGAC consortium to publish open-access repositories of polygenic indices, the use of genetic data in social science datasets is becoming increasingly accessible and user-friendly \citep{okbay2019repository}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\section{The relevance of \texorpdfstring{$G \times E$}{} interplay}\label{sec:why}
The study of the interplay between `nature' (genetic endowments) and `nurture' (environmental conditions) has a long history in the social sciences \citep[e.g.,][]{Haldane1946, Plomin1977, Caspi2002, Caspi2003, Guo2002, Dickens2001, Ridley2003, Rutter2006gxereview, Khoury2017}. These earlier accounts were largely philosophical and/or theoretical since large-scale measurement of genetic data was not possible until the completion of the Human Genome Project in the early 2000s. We seek to (1) familiarize the reader to key concepts and developments in the field of $G \times E$ interplay and (2) offer practical guidance to empirical researchers who aim to integrate publicly available PGIs in their models. Our study builds upon and extends general surveys on the promise of using genetic data in economic analyses such as found in \citet{Benjamin2011} and \citet{Beauchamp2011} %\citet{lehrer2017genetic}
and more specifically surveys on $G \times E$ in \citet{Fletcher2013} and \citet{Schmitz2017}.\footnote{See \cite{Rutter2006}, \citet{Plomin2014}, \citet{Mills2020book} and \citet{domingue2020interactions} for closely related work in other disciplines.}

This paper updates and extends the scope of these previous efforts, presents a theoretical framework to guide and interpret empirical analyses, and intends to be a practitioner's guide for applied researchers interested in using genetic data in their research. The running example we employ throughout the paper uses educational attainment as the main outcome, and we study the interplay between the polygenic index for educational attainment and various environmental conditions. In particular, in our empirical illustration in \hyperref[sec:application]{Section~\ref*{sec:application}} we show how month of birth interacts with genetic endowments in influencing children's test scores in the UK. To dispel any doubts about the scientific and policy relevance of gene-by-environment interplay, we first address the question of why it is important to realize our two aims, and why \textit{now} is the time to realize them.

\textit{Why is it important to realize our goals?}
First, and arguably foremost, improved understanding of $G \times E$ interplay represents a basic scientific advance in our understanding of how nature and nurture interact in shaping human capabilities. This in turn may lead to unforeseen advances in scientific knowledge as well as to novel applications. More specifically, an important part of (micro-)economics is the study of human (economic) behavior and social and economic outcomes. Differences in genetic makeup play a substantial role in such outcomes. For example, twin studies suggest that some 25-75\% of the variation between individuals for a wide range of (economic) behaviors, traits, health and socio-economic outcomes, can be attributed to genetic differences between individuals \citep[see, e.g.,][]{Polderman2015}. In fact, the large body of evidence stemming from heritability studies has been synthesized into the first law of behavior genetics stating that ``\textit{all human behavioural traits are heritable}'' \citep{Turkheimer2000}. With recent advances in the analysis and collection of genetic data, we believe that economists can no longer ignore the significant role of genetic variation in their analyses.

Second, the study of $G \times E$ provides novel ways of testing economic theories and mechanisms. For example, the concept of dynamic complementarity stipulates that skills produced at one stage raise the productivity of later investments \citep[e.g.,][]{cunha2007technology}. However, testing for dynamic complementarity in skill formation is notoriously challenging, since it requires independent variation in initial endowments and subsequent investments, or, alternatively, exogenous variation in sequential investments over time \citep{almond2018childhood,johnson2019reducing}. In practice, measures of children’s endowments (e.g., birth weight) are rarely clean of parental investments, and parental investments are serially correlated over time, posing a formidable empirical challenge to accurately identify dynamic complementarities in skill formation. Genetic data has the major advantage that it is fixed at conception and invariant over the life cycle, and therefore insensitive to (parental) behavior. Studying how parental investments \citep{Muslimova2020b} or public policies \citep{barth2020genetic} influence the relationship between genes and economic outcomes is therefore highly relevant to better understand the production function for skills and wealth accumulation.

Although the exact mechanism through which the interplay between genes and environments shapes human behavior is currently not well understood, it is likely to represent a non-negligible source of variation in human behavior, traits, and other outcomes. Forestry research provides an interesting analogy here. The genetic propensity of a tree to grow big (in terms of height, volume, etc.) is sizeable, with heritabilities ranging from 30 to 60\% for tree height and size \citep{st1994genetic}. This is comparable to the heritability of anthropomorphic traits for humans \citep[48\% for height and 22\% for weight,][]{Yengo2018}. But Bonzai artisans can completely negate the genetic propensity of trees to become large. By carefully controlling its environment the Bonzai tree never reaches the size of its family members in the forest, illustrating the substantial role that the environment can have%\footnote{Bonzai trees can live very long lives, with several trees known to be older than 1,000 years, suggesting that they are in fact quite healthy and that life is capable of adjusting optimally to different circumstances.}
Indeed, returning to humans, environmental conditions, in particular those early in life, can have long-lasting and sometimes irreversible effects on life outcomes \citep[e.g.,][]{campbell2014early,almond2018childhood}. These results suggest that $G \times E$ interplay studies have great potential for improving our understanding of the substantial variation observed in human capabilities across individuals. With that, they can help inform the (public) discussion around genetic or environmental determinism \citep{schnittker2015gene}.

Finally, although there has been a heated debate about the policy-relevance of heritability studies \citep{Goldberger1979,taubman1981heritability,Manski2011}, the study of $G \times E$ interplay can contribute novel evidence for policy makers. For example, it may become possible to identify environments or policies that reduce or even neutralize genetic inequalities, or that help individuals better reach their genetic potential \citep{Bierut2018}. Although the current predictive power of genetic indices precludes \textit{individual} prediction of future traits such as disease outcomes, it performs well at the \textit{group}- or \textit{population}-level. Understanding how environmental exposures affect social or economic outcomes for different genetically at risk groups may be useful to policy makers. For example, genetic information could then be used preventatively by informing individuals (e.g., by a medical doctor) to avoid environments that may harm them. The validity of such policy recommendations stemming from empirical studies crucially hinges on the correct specification and interpretation of empirical models. In this study, we provide a guide to empirical researchers, discussing this in detail.

%Interestingly, observing genetic data has the potential to neutralize genetic disadvantage even before the actual outcome is realized. For example, it is possible to measure one's genetic predisposition for Alzheimer's disease or the risk of developing ADHD already at birth. Studying which environmental responses prevent people with higher risk for ADHD or Alzheimer's disease from developing actual symptoms or disease could bring huge benefit to the affected individuals.
%\textit{How can economists contribute to and benefit from the realization of these two goals?} First, economics studies how individuals respond to constraints and incentives. There is abundant evidence that one's genetic make-up influences lifecycle choices, such as smoking \citep{Erzurumluoglu2019}, alcohol consumption \citep{kranzler2019}, food intake \citep{Meddens2020}, and risk taking \citep{KarlssonLinner2019}. Economic theories can help understand and predict these individual choices. When specified within an economic framework, studies of gene-by-environment interplay can aid the interpretation of economic parameters and improve our understanding of unobserved, as well as observed, heterogeneity \citep{Biroli2015,Benjamin2014}. As such, the availability of genetic data provides a new frontier in the measurement of potentially relevant treatment effect heterogeneity. Heterogeneity of treatment effects by genotype is not merely important to better understand the effectiveness of targeted policies (as with any heterogeneity in treatment effects), but additionally has important intergenerational implications. For example, if a certain social policy consistently fails to have its intended effect on a target group with a specific genetic predisposition, then this policy failure may propagate across generations (as genes are passed on to offspring), potentially increasing intergenerational inequalities.

%Second, recognizing that the environments that individuals self-select into are partially shaped by incentives and (genetic) constraints, it is clear that the study of $G \times E$ interplay is subject to endogeneity concerns. In fact, as we will argue below, not taking into account the endogenous nature of both $G$ and $E$ will lead to biased estimates and parameters that are very difficult to interpret. Economists have substantial experience with exploiting exogenous variation in environmental (and other) exposures and have developed a large toolbox to dealing with endogeneity. Given the importance of establishing which causal environmental exposures moderate what genetic risk, economists are well-positioned to improving understanding of the complex interplay between genes and the environment in shaping life outcomes.

\textit{Why is now the time to realize our goals?}
Recent technological advances in the mapping of the genome, rapid reductions in the costs of measuring genetic variation across people, and fast growth in sample sizes have led to substantial growth in the power of genetic discovery studies, also known as genome-wide association studies (GWAS).\footnote{See \hyperref[sec:G]{Section~\ref*{sec:G}} for a detailed discussion of GWAS and \hyperref[sec:glossary]{Appendix~\ref*{sec:glossary}} for a glossary.} Economists have been pioneers in pushing the GWAS approach to uncover the genetic underpinnings of a range of social and economic outcomes, such as educational attainment \citep{Rietveld2013,Okbay2016,lee2018gene}, subjective well-being \citep{Okbay2016well}, and risk aversion \citep{KarlssonLinner2019}. These GWAS discovery studies have enabled researchers to construct highly predictive polygenic indices (PGIs) that summarize the effects of multiple genetics variants. For example, the PGI for educational attainment, constructed on the basis of the latest GWAS, has a predictive power ($R^2$) of $\sim$12\% in an independent hold-out sample, making its effects detectable with 80\% power at a $p$-value threshold of 0.05 in a sample of only 70 individuals \citep{lee2018gene}.\footnote{This is a substantial improvement over the use of individual SNPs. For example, the SNP most strongly associated with educational attainment has an $R^2$ of only $\sim$0.02\% %, equivalent to approximately 1 month of schooling per ``allele''
\citep{Rietveld2013,Okbay2016}.} Today, results of GWASs are available for hundreds of human traits (see e.g., https://atlas.ctglab.nl/) making it possible to study $G \times E$ interplay in these traits, even in studies of relatively small size by using the power of polygenic indices.

Polygenic indices are now available or can be constructed in several datasets commonly used by economists.\footnote{Examples of such datasets include the Avon Longitudinal Study of Parents and Children (ALSPAC), the German Socioeconomic Panel (GSOEP), the National Longitudinal Study of Adolescent to Adult Health (AddHealth), the English Longitudinal Study of Ageing (ELSA), the Framingham Heart Study (FHS), the Health and Retirement Study (HRS), the Millenium Cohort Study (MCS), the National Child Development Study (NCDS), the National Survey of Health and Development Cohort (NSHD), the UK Household Longitudinal Study (UKHLS, `Understanding Society'), the UK Biobank (UKB), and the Wisconsin Longitudinal Study (WLS).} Until recently, accessing and processing the genetic data in these surveys required specific software and skills. With the progress in polygenic prediction, and the efforts of, e.g., the Health and Retirement Study and the SSGAC consortium to publish open-access repositories of polygenic indices, the use of genetic data in social science datasets is becoming increasingly accessible and user-friendly \citep{okbay2019repository}. Economists and other social scientists have started to leverage these developments by demonstrating the different ways in which genetic information can be used to answer economic and social science research questions \citep[e.g.,][]{Belsky2018mobility,Domingue2015a,Domingue2018,barth2020genetic,papageorge2020genes,rietveld2016genetic,Turley2018,Barcellos2018,VonHinke2013,VonHinke2014,VonHinke2016,Muslimova2020b,pereira2020interplay}. The growing interest in genoeconomics, and its coming to maturity, is reflected in the fact that such studies are getting published in journals such as \textit{Nature}, \textit{Nature Genetics}, the \textit{Journal of Political Economy}, the \textit{Journal of the European Economic Association}, and the \textit{Proceedings of the National Academy of Sciences}.

However, these developments also pose a number of challenges on the best empirical specification as well as the interpretation of the estimates of $G \times E$ interplay. This is particularly true for economists who are not (yet) familiar with the underlying genetic data and research. These readily available polygenic indices could therefore easily be applied na\"ively or misinterpreted in some way. It is therefore timely and essential to highlight the challenges in the estimation of $G \times E$ interplay and to discuss the proper interpretation of such estimates.


==> Scraps.tex <==
It is useful to contrast the decomposition in Equation (\ref{eq:GEDecomp}) with other lists of \textit{G $\times$ E} interplay mechanisms described in the literature.  In particular, \citet{shanahan2005social} offer the following taxonomy of four, non-mutually exclusive mechanisms through which environments or social context can moderate the relationship between genes and outcomes:
\begin{enumerate} 
\item	Contextual triggering: social context acts as a stressor that activates (or ``triggers'') one’s genetic disposition (e.g., life events trigger genetic disposition towards depression).
\item	Compensation: an enriched social context (or simply the absence of a trigger) prevents/neutralizes the expression of one's genetic predisposition (in some sense, this is the other end of the spectrum compared with contextual triggering). 
\item	Social control: social norms and / or other forces restrict the genetic propensity to certain traits (e.g., social norms limiting one's genetic propensity to alcohol consumption or one's genetic propensity to having first intercourse at a young age).
\item	Enhancement: social context enhances  genetic predispositions (e.g., education reforms may reinforce genetic potential for educational attainment).
\end{enumerate}

The interactions described here have analogues to the terms in Equation (\ref{eq:GEDecomp}).  For example, one could consider \textit{contextual triggering} to be a case of technological $GxE$ with $F_{G}<0$ and $F_{GE}<0$, while \textit{contextual compensation} corresponds to the case where $F_{G}<0$ and $F_{GE}>0$.  The concepts of \textit{social control} and \textit{social enhancement} could refer to numerous configurations of ...

==> include/MoB_all_outcomes.tex <==
            &\multicolumn{2}{c}{Entry Assessment}       &\multicolumn{2}{c}{Key Stage 1}            &\multicolumn{2}{c}{Key Stage 2}            &\multicolumn{2}{c}{Key Stage 3}            &\multicolumn{2}{c}{Key Stage 4}            \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
\midrule
Treated     &       1.138\sym{***}&       1.133\sym{***}&       0.712\sym{***}&       0.698\sym{***}&       0.392\sym{***}&       0.389\sym{***}&       0.226\sym{***}&       0.223\sym{**} &       0.285\sym{***}&       0.281\sym{***}\\
            &     (0.088)         &     (0.077)         &     (0.024)         &     (0.026)         &     (0.021)         &     (0.021)         &     (0.055)         &     (0.057)         &     (0.023)         &     (0.021)         \\
\addlinespace
PGI         &       0.155\sym{***}&       0.024         &       0.261\sym{***}&       0.315\sym{***}&       0.347\sym{***}&       0.366\sym{***}&       0.358\sym{***}&       0.320\sym{***}&       0.318\sym{***}&       0.346\sym{***}\\
            &     (0.027)         &     (0.024)         &     (0.016)         &     (0.002)         &     (0.011)         &     (0.019)         &     (0.015)         &     (0.015)         &     (0.008)         &     (0.004)         \\
\addlinespace
Treated*PGI &                     &       0.087\sym{*}  &                     &      -0.087\sym{**} &                     &      -0.052\sym{*}  &                     &       0.011         &                     &      -0.050\sym{***}\\
            &                     &     (0.035)         &                     &     (0.026)         &                     &     (0.023)         &                     &     (0.022)         &                     &     (0.010)         \\
\addlinespace
Treated*MoB &       0.055         &       0.059         &       0.054\sym{***}&       0.049\sym{**} &       0.085\sym{***}&       0.080\sym{***}&       0.019         &       0.018         &       0.023         &       0.019         \\
            &     (0.045)         &     (0.045)         &     (0.013)         &     (0.013)         &     (0.012)         &     (0.011)         &     (0.029)         &     (0.032)         &     (0.013)         &     (0.012)         \\
\addlinespace
MoB*PGI     &                     &      -0.080\sym{**} &                     &       0.040\sym{***}&                     &       0.011         &                     &      -0.013         &                     &       0.020\sym{***}\\
            &                     &     (0.021)         &                     &     (0.002)         &                     &     (0.013)         &                     &     (0.012)         &                     &     (0.003)         \\
\addlinespace
MoB*PGI*Treated&                     &       0.127\sym{***}&                     &      -0.011         &                     &       0.015         &                     &       0.047\sym{***}&                     &      -0.002         \\
            &                     &     (0.025)         &                     &     (0.012)         &                     &     (0.012)         &                     &     (0.011)         &                     &     (0.010)         \\
\midrule
R2          &       0.258         &       0.267         &       0.175         &       0.182         &       0.147         &       0.151         &       0.147         &       0.149         &       0.142         &       0.145         \\
Observations&        1094         &        1094         &        3436         &        3436         &        3610         &        3610         &        3073         &        3073         &        3579         &        3579         \\


==> include/MoB_ks1.tex <==
            &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Treated     &       0.712\sym{***}&       0.698\sym{***}\\
            &     (0.024)         &     (0.026)         \\
\addlinespace
PGI         &       0.261\sym{***}&       0.315\sym{***}\\
            &     (0.016)         &     (0.002)         \\
\addlinespace
Treated*PGI &                     &      -0.087\sym{**} \\
            &                     &     (0.026)         \\
\addlinespace
Treated*MoB &       0.054\sym{***}&       0.049\sym{**} \\
            &     (0.013)         &     (0.013)         \\
\addlinespace
MoB*PGI     &                     &       0.040\sym{***}\\
            &                     &     (0.002)         \\
\addlinespace
MoB*PGI*Treated&                     &      -0.011         \\
            &                     &     (0.012)         \\
\midrule
R2          &       0.175         &       0.182         \\
Observations&        3436         &        3436         \\


==> include/MoB_ks2.tex <==
            &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Treated     &       0.392\sym{***}&       0.389\sym{***}\\
            &     (0.021)         &     (0.021)         \\
\addlinespace
PGI         &       0.347\sym{***}&       0.366\sym{***}\\
            &     (0.011)         &     (0.019)         \\
\addlinespace
Treated*PGI &                     &      -0.052\sym{*}  \\
            &                     &     (0.023)         \\
\addlinespace
Treated*MoB &       0.085\sym{***}&       0.080\sym{***}\\
            &     (0.012)         &     (0.011)         \\
\addlinespace
MoB*PGI     &                     &       0.011         \\
            &                     &     (0.013)         \\
\addlinespace
MoB*PGI*Treated&                     &       0.015         \\
            &                     &     (0.012)         \\
\midrule
R2          &       0.147         &       0.151         \\
Observations&        3610         &        3610         \\


==> include/MoB_ks3.tex <==
            &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Treated     &       0.226\sym{***}&       0.223\sym{**} \\
            &     (0.055)         &     (0.057)         \\
\addlinespace
PGI         &       0.358\sym{***}&       0.320\sym{***}\\
            &     (0.015)         &     (0.015)         \\
\addlinespace
Treated*PGI &                     &       0.011         \\
            &                     &     (0.022)         \\
\addlinespace
Treated*MoB &       0.019         &       0.018         \\
            &     (0.029)         &     (0.032)         \\
\addlinespace
MoB*PGI     &                     &      -0.013         \\
            &                     &     (0.012)         \\
\addlinespace
MoB*PGI*Treated&                     &       0.047\sym{***}\\
            &                     &     (0.011)         \\
\midrule
R2          &       0.147         &       0.149         \\
Observations&        3073         &        3073         \\


==> include/MoB_ks4.tex <==
            &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Treated     &       0.285\sym{***}&       0.281\sym{***}\\
            &     (0.023)         &     (0.021)         \\
\addlinespace
PGI         &       0.318\sym{***}&       0.346\sym{***}\\
            &     (0.008)         &     (0.004)         \\
\addlinespace
Treated*PGI &                     &      -0.050\sym{***}\\
            &                     &     (0.010)         \\
\addlinespace
Treated*MoB &       0.023         &       0.019         \\
            &     (0.013)         &     (0.012)         \\
\addlinespace
MoB*PGI     &                     &       0.020\sym{***}\\
            &                     &     (0.003)         \\
\addlinespace
MoB*PGI*Treated&                     &      -0.002         \\
            &                     &     (0.010)         \\
\midrule
R2          &       0.142         &       0.145         \\
Observations&        3579         &        3579         \\


==> include/ORIV_all.tex <==
            &  Entry Ass.         & Key Stage 1         & Key Stage 2         & Key Stage 3         & Key Stage 4         \\
\midrule
Treated     &       1.135\sym{***}&       0.720\sym{***}&       0.410\sym{***}&       0.243\sym{***}&       0.305\sym{***}\\
            &     (0.076)         &     (0.052)         &     (0.060)         &     (0.055)         &     (0.030)         \\
\addlinespace
PGI         &       0.068\sym{**} &       0.371\sym{***}&       0.414\sym{***}&       0.365\sym{***}&       0.390\sym{***}\\
            &     (0.017)         &     (0.009)         &     (0.017)         &     (0.018)         &     (0.009)         \\
\addlinespace
Treated $\times$ PGI &       0.064\sym{***}&      -0.082\sym{*}  &      -0.020         &       0.050         &      -0.010         \\
            &     (0.013)         &     (0.038)         &     (0.033)         &     (0.032)         &     (0.010)         \\
\addlinespace
%Treated*MoB &                     &                     &                     &                     &                     \\
%            &                     &                     &                     &                     &                     \\
%\addlinespace
MoB $\times$ PGI     &      -0.076\sym{***}&       0.050\sym{***}&       0.003         &      -0.018         &       0.012         \\
            &     (0.018)         &     (0.004)         &     (0.011)         &     (0.013)         &     (0.006)         \\
\addlinespace
MoB $\times$ PGI $\times$ Treated&       0.139\sym{***}&      -0.017         &       0.025\sym{*}  &       0.068\sym{***}&       0.006         \\
            &     (0.031)         &     (0.015)         &     (0.012)         &     (0.010)         &     (0.016)         \\
\addlinespace
MoB         &      -0.118\sym{***}&      -0.064\sym{***}&      -0.063\sym{**} &      -0.020         &      -0.033\sym{***}\\
            &     (0.027)         &     (0.012)         &     (0.020)         &     (0.014)         &     (0.008)         \\
\midrule
$1^{st}$ stage $F$-stat&    2663         &    2663         &    2663         &    2663         &    2663         \\
Observations&        1094         &        3436         &        3610         &        3073         &        3579         \\


==> include/PredictivePower_ea.tex <==
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
PGI plink           &       0.157\sym{***}&                     &                     &                     \\
                    &     (0.029)         &                     &                     &                     \\
\addlinespace
PGI ukb             &                     &       0.161\sym{***}&                     &                     \\
                    &                     &     (0.029)         &                     &                     \\
\addlinespace
PGI 23me            &                     &                     &       0.121\sym{***}&                     \\
                    &                     &                     &     (0.029)         &                     \\
\addlinespace
PGI 23me\_ukb        &                     &                     &                     &       0.163\sym{***}\\
                    &                     &                     &                     &     (0.028)         \\
\midrule
R2                  &       0.081         &       0.083         &       0.073         &       0.085         \\
Observations        &        1094         &        1094         &        1094         &        1094         \\


==> include/PredictivePower_ks1.tex <==
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
PGI plink           &       0.231\sym{***}&                     &                     &                     \\
                    &     (0.015)         &                     &                     &                     \\
\addlinespace
PGI ukb             &                     &       0.253\sym{***}&                     &                     \\
                    &                     &     (0.015)         &                     &                     \\
\addlinespace
PGI 23me            &                     &                     &       0.205\sym{***}&                     \\
                    &                     &                     &     (0.016)         &                     \\
\addlinespace
PGI 23me\_ukb        &                     &                     &                     &       0.255\sym{***}\\
                    &                     &                     &                     &     (0.015)         \\
\midrule
R2                  &       0.085         &       0.096         &       0.072         &       0.096         \\
Observations        &        3436         &        3436         &        3436         &        3436         \\


==> include/PredictivePower_ks2.tex <==
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
PGI plink           &       0.289\sym{***}&                     &                     &                     \\
                    &     (0.015)         &                     &                     &                     \\
\addlinespace
PGI ukb             &                     &       0.319\sym{***}&                     &                     \\
                    &                     &     (0.015)         &                     &                     \\
\addlinespace
PGI 23me            &                     &                     &       0.286\sym{***}&                     \\
                    &                     &                     &     (0.015)         &                     \\
\addlinespace
PGI 23me\_ukb        &                     &                     &                     &       0.344\sym{***}\\
                    &                     &                     &                     &     (0.015)         \\
\midrule
R2                  &       0.092         &       0.112         &       0.089         &       0.128         \\
Observations        &        3610         &        3610         &        3610         &        3610         \\


==> include/PredictivePower_ks3.tex <==
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
PGI plink           &       0.313\sym{***}&                     &                     &                     \\
                    &     (0.017)         &                     &                     &                     \\
\addlinespace
PGI ukb             &                     &       0.331\sym{***}&                     &                     \\
                    &                     &     (0.017)         &                     &                     \\
\addlinespace
PGI 23me            &                     &                     &       0.303\sym{***}&                     \\
                    &                     &                     &     (0.017)         &                     \\
\addlinespace
PGI 23me\_ukb        &                     &                     &                     &       0.357\sym{***}\\
                    &                     &                     &                     &     (0.017)         \\
\midrule
R2                  &       0.107         &       0.117         &       0.097         &       0.134         \\
Observations        &        3073         &        3073         &        3073         &        3073         \\


==> include/PredictivePower_ks4.tex <==
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
PGI plink           &       0.274\sym{***}&                     &                     &                     \\
                    &     (0.016)         &                     &                     &                     \\
\addlinespace
PGI ukb             &                     &       0.293\sym{***}&                     &                     \\
                    &                     &     (0.016)         &                     &                     \\
\addlinespace
PGI 23me            &                     &                     &       0.274\sym{***}&                     \\
                    &                     &                     &     (0.015)         &                     \\
\addlinespace
PGI 23me\_ukb        &                     &                     &                     &       0.318\sym{***}\\
                    &                     &                     &                     &     (0.016)         \\
\midrule
R2                  &       0.103         &       0.113         &       0.101         &       0.128         \\
Observations        &        3579         &        3579         &        3579         &        3579         \\


==> include/corr_treat_PGS.tex <==
            &\multicolumn{1}{c}{(1)}         \\
\midrule
Child PGI   &       0.002         \\
            &     (0.012)         \\
\addlinespace
Mom PGI     &       0.004         \\
            &     (0.005)         \\
\midrule
R2          &       0.016         \\
Observations&        3059         \\


==> include_OLD/DescrByTreated.tex <==
%\midrule
Mother's age at first pregnancy&        2,062&      25.138&            &        2168&      25.257&            &        4,230&            &       0.431\\
Mother smoked cigarettes during pregnancy&        1,927&       0.167&            &        2052&       0.168&            &        3,979&            &       0.896\\
Mother's anxiety score during pregnancy&        1,888&       4.651&            &        2,037&       4.659&            &        3925&            &       0.946\\
Mother's depression score during pregnancy&        1,887&       4.245&            &        2,038&       4.211&            &        3925&            &       0.714\\
Mother is married   &        2,061&       0.843&            &        2169&       0.859&            &        4,230&            &       0.153\\
Mother proportion vocational&        2,047&       0.096&            &        2146&       0.088&            &        4193&            &       0.361\\
Mother proportion O-level&        2,047&       0.338&            &        2,146&       0.366&            &        4,193&            &       0.056\\
Mother proportion A-level&        2047&       0.248&            &        2,146&       0.241&            &        4,193&            &       0.609\\
Mother proportion Degree&        2047&       0.157&            &        2,146&       0.156&            &        4,193&            &       0.882\\
Partner proportion vocational&        1,976&       0.082&            &        2085&       0.071&            &        4,061&            &       0.188\\
Partner proportion O-level&        1976&       0.197&            &        2,085&       0.218&            &        4061&            &       0.101\\
Partner proportion A-level&        1976&       0.275&            &        2085&       0.278&            &        4061&            &       0.836\\
Partner proportion Degree&        1976&       0.214&            &        2085&       0.228&            &        4061&            &       0.258\\
Mother proportion Social Class II&        1713&       0.325&            &        1864&       0.326&            &        3577&            &       0.948\\
Mother proportion Social Class III(non-manual)&        1713&       0.422&            &        1864&       0.434&            &        3577&            &       0.471\\
Mother proportion Social Class III(manual)&        1713&       0.067&            &        1864&       0.072&            &        3577&            &       0.576\\
Mother proportion Social Class IV&        1713&       0.101&            &        1864&       0.083&            &        3577&            &       0.058\\
Mother proportion Social Class V&        1713&       0.016&            &        1864&       0.014&            &        3577&            &       0.652\\
Child's birthweight (in g)&        2089&    3448.347&            &        2189&    3450.876&            &        4278&            &       0.875\\
Child PGI for Educational Attainment&        2114&       0.016&            &        2209&       0.037&            &        4323&            &       0.499\\
Mother PGI for Educational Attainment&        1526&       0.036&            &        1533&       0.022&            &        3059&            &       0.688\\


==> include_OLD/MoB_ea.tex <==
            &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Treated     &       1.041\sym{***}&       1.022\sym{***}\\
            &     (0.070)         &     (0.073)         \\
\addlinespace
Treated$\times$PGI &                     &      -0.264\sym{***}\\
            &                     &     (0.040)         \\
\addlinespace
Treated$\times$MoB &       0.056         &       0.064         \\
            &     (0.050)         &     (0.055)         \\
\addlinespace
MoB$\times$PGI     &                     &      -0.088\sym{***}\\
            &                     &     (0.002)         \\
\addlinespace
MoB$\times$PGI$\times$Treated&                     &       0.166\sym{***}\\
            &                     &     (0.015)         \\
\addlinespace
MoB         &      -0.140\sym{**} &      -0.141\sym{**} \\
            &     (0.050)         &     (0.049)         \\
\addlinespace
PGI         &       0.159\sym{***}&       0.206\sym{***}\\
            &     (0.036)         &     (0.032)         \\
\midrule
R2          &       0.246         &       0.258         \\
Observations&        1094         &        1094         \\


==> include_OLD/MoB_ea_23me.tex <==
            &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Treated     &       1.052\sym{***}&       0.882\sym{***}\\
            &     (0.064)         &     (0.057)         \\
\addlinespace
Treated*PGI &                     &      -0.145\sym{**} \\
            &                     &     (0.051)         \\
\addlinespace
Treated*MoB &       0.054         &       0.077         \\
            &     (0.045)         &     (0.047)         \\
\addlinespace
MoB*PGI     &                     &      -0.047\sym{**} \\
            &                     &     (0.015)         \\
\addlinespace
MoB*PGI*Treated&                     &       0.106\sym{***}\\
            &                     &     (0.025)         \\
\addlinespace
MoB         &      -0.141\sym{**} &      -0.158\sym{**} \\
            &     (0.046)         &     (0.043)         \\
\addlinespace
PGI         &       0.119\sym{***}&       0.126\sym{***}\\
            &     (0.025)         &     (0.024)         \\
\midrule
R2          &       0.237         &       0.251         \\
Observations&        1094         &        1094         \\


==> include_OLD/MoB_ea_23me_ukb.tex <==
            &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Treated     &       1.057\sym{***}&       0.892\sym{***}\\
            &     (0.073)         &     (0.068)         \\
\addlinespace
Treated*PGI &                     &      -0.099         \\
            &                     &     (0.056)         \\
\addlinespace
Treated*MoB &       0.047         &       0.061         \\
            &     (0.044)         &     (0.045)         \\
\addlinespace
MoB*PGI     &                     &      -0.078\sym{**} \\
            &                     &     (0.022)         \\
\addlinespace
MoB*PGI*Treated&                     &       0.130\sym{***}\\
            &                     &     (0.030)         \\
\addlinespace
MoB         &      -0.138\sym{**} &      -0.146\sym{**} \\
            &     (0.045)         &     (0.041)         \\
\addlinespace
PGI         &       0.157\sym{***}&       0.148\sym{***}\\
            &     (0.029)         &     (0.033)         \\
\midrule
R2          &       0.248         &       0.261         \\
Observations&        1094         &        1094         \\


==> include_OLD/MoB_ea_plink.tex <==
            &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Treated     &       1.054\sym{***}&       0.859\sym{***}\\
            &     (0.074)         &     (0.065)         \\
\addlinespace
Treated*PGI &                     &      -0.280\sym{***}\\
            &                     &     (0.048)         \\
\addlinespace
Treated*MoB &       0.058         &       0.083         \\
            &     (0.049)         &     (0.056)         \\
\addlinespace
MoB*PGI     &                     &      -0.084\sym{***}\\
            &                     &     (0.010)         \\
\addlinespace
MoB*PGI*Treated&                     &       0.162\sym{***}\\
            &                     &     (0.019)         \\
\addlinespace
MoB         &      -0.144\sym{**} &      -0.156\sym{**} \\
            &     (0.050)         &     (0.049)         \\
\addlinespace
PGI         &       0.164\sym{***}&       0.193\sym{***}\\
            &     (0.037)         &     (0.029)         \\
\midrule
R2          &       0.248         &       0.264         \\
Observations&        1094         &        1094         \\


==> include_OLD/MoB_ea_ukb.tex <==
            &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\midrule
Treated     &       1.055\sym{***}&       0.889\sym{***}\\
            &     (0.080)         &     (0.084)         \\
\addlinespace
Treated*PGI &                     &      -0.090         \\
            &                     &     (0.078)         \\
\addlinespace
Treated*MoB &       0.057         &       0.066         \\
            &     (0.047)         &     (0.049)         \\
\addlinespace
MoB*PGI     &                     &      -0.066\sym{***}\\
            &                     &     (0.015)         \\
\addlinespace
MoB*PGI*Treated&                     &       0.106\sym{**} \\
            &                     &     (0.030)         \\
\addlinespace
MoB         &      -0.146\sym{**} &      -0.145\sym{**} \\
            &     (0.046)         &     (0.043)         \\
\addlinespace
PGI         &       0.161\sym{***}&       0.161\sym{**} \\
            &     (0.024)         &     (0.059)         \\
\midrule
R2          &       0.247         &       0.260         \\
Observations&        1094         &        1094         \\


==> include_OLD/MoB_ks.tex <==
            &\multicolumn{2}{c}{Key Stage 1}            &\multicolumn{2}{c}{Key Stage 2}            &\multicolumn{2}{c}{Key Stage 3}            &\multicolumn{2}{c}{Key Stage 4}            \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\midrule
Treated     &       0.597\sym{***}&       0.589\sym{***}&       0.212\sym{***}&       0.217\sym{***}&       0.141         &       0.126         &       0.193\sym{***}&       0.198\sym{***}\\
            &     (0.016)         &     (0.019)         &     (0.016)         &     (0.018)         &     (0.081)         &     (0.078)         &     (0.032)         &     (0.034)         \\
\addlinespace
Treated$\times$PGI &                     &      -0.092\sym{**} &                     &      -0.057\sym{*}  &                     &      -0.092\sym{***}&                     &      -0.015         \\
            &                     &     (0.027)         &                     &     (0.028)         &                     &     (0.017)         &                     &     (0.014)         \\
\addlinespace
Treated$\times$MoB &       0.072\sym{***}&       0.072\sym{***}&       0.108\sym{***}&       0.108\sym{***}&       0.045         &       0.051         &       0.049\sym{**} &       0.050\sym{**} \\
            &     (0.012)         &     (0.010)         &     (0.013)         &     (0.012)         &     (0.030)         &     (0.031)         &     (0.014)         &     (0.015)         \\
\addlinespace
MoB$\times$PGI     &                     &       0.018\sym{**} &                     &       0.006         &                     &       0.034\sym{***}&                     &       0.048\sym{***}\\
            &                     &     (0.006)         &                     &     (0.010)         &                     &     (0.005)         &                     &     (0.007)         \\
\addlinespace
MoB$\times$PGI$\times$Treated&                     &       0.011         &                     &       0.016         &                     &       0.013         &                     &      -0.039\sym{**} \\
            &                     &     (0.010)         &                     &     (0.013)         &                     &     (0.007)         &                     &     (0.010)         \\
\addlinespace
MoB         &      -0.095\sym{***}&      -0.093\sym{***}&      -0.098\sym{***}&      -0.099\sym{***}&      -0.029         &      -0.030\sym{*}  &      -0.045\sym{**} &      -0.047\sym{***}\\
            &     (0.010)         &     (0.011)         &     (0.011)         &     (0.010)         &     (0.015)         &     (0.014)         &     (0.011)         &     (0.011)         \\
\addlinespace
PGI         &       0.237\sym{***}&       0.205\sym{***}&       0.291\sym{***}&       0.262\sym{***}&       0.314\sym{***}&       0.295\sym{***}&       0.275\sym{***}&       0.258\sym{***}\\
            &     (0.011)         &     (0.023)         &     (0.010)         &     (0.013)         &     (0.017)         &     (0.017)         &     (0.013)         &     (0.015)         \\
\midrule
R2          &       0.158         &       0.163         &       0.110         &       0.112         &       0.115         &       0.118         &       0.113         &       0.117         \\
Observations&        3436         &        3436         &        3610         &        3610         &        3073         &        3073         &        3579         &        3579         \\


==> include_OLD/MoB_ks_23me.tex <==
            &\multicolumn{2}{c}{Key Stage 1}            &\multicolumn{2}{c}{Key Stage 2}            &\multicolumn{2}{c}{Key Stage 3}            &\multicolumn{2}{c}{Key Stage 4}            \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\midrule
Treated     &       0.620\sym{***}&       0.658\sym{***}&       0.262\sym{***}&       0.202\sym{***}&       0.188         &       0.243\sym{**} &       0.241\sym{***}&       0.263\sym{***}\\
            &     (0.019)         &     (0.046)         &     (0.031)         &     (0.031)         &     (0.098)         &     (0.083)         &     (0.043)         &     (0.041)         \\
\addlinespace
Treated*PGI &                     &      -0.112\sym{**} &                     &      -0.069\sym{***}&                     &      -0.049\sym{**} &                     &      -0.041         \\
            &                     &     (0.038)         &                     &     (0.008)         &                     &     (0.016)         &                     &     (0.025)         \\
\addlinespace
Treated*MoB &       0.056\sym{***}&       0.052\sym{**} &       0.082\sym{***}&       0.081\sym{***}&       0.015         &       0.009         &       0.023         &       0.021         \\
            &     (0.012)         &     (0.014)         &     (0.016)         &     (0.015)         &     (0.036)         &     (0.036)         &     (0.018)         &     (0.018)         \\
\addlinespace
MoB*PGI     &                     &       0.048\sym{***}&                     &       0.012         &                     &       0.009         &                     &       0.022\sym{***}\\
            &                     &     (0.012)         &                     &     (0.010)         &                     &     (0.007)         &                     &     (0.003)         \\
\addlinespace
MoB*PGI*Treated&                     &      -0.006         &                     &       0.012         &                     &       0.037\sym{***}&                     &      -0.003         \\
            &                     &     (0.015)         &                     &     (0.009)         &                     &     (0.005)         &                     &     (0.011)         \\
\addlinespace
MoB         &      -0.087\sym{***}&      -0.083\sym{***}&      -0.091\sym{***}&      -0.092\sym{***}&      -0.016         &      -0.014         &      -0.033\sym{**} &      -0.033\sym{**} \\
            &     (0.012)         &     (0.013)         &     (0.012)         &     (0.009)         &     (0.015)         &     (0.013)         &     (0.012)         &     (0.011)         \\
\addlinespace
PGI         &       0.210\sym{***}&       0.197\sym{***}&       0.287\sym{***}&       0.275\sym{***}&       0.304\sym{***}&       0.253\sym{***}&       0.274\sym{***}&       0.249\sym{***}\\
            &     (0.020)         &     (0.013)         &     (0.010)         &     (0.024)         &     (0.021)         &     (0.023)         &     (0.007)         &     (0.019)         \\
\midrule
R2          &       0.149         &       0.153         &       0.106         &       0.108         &       0.106         &       0.110         &       0.113         &       0.116         \\
Observations&        3436         &        3436         &        3610         &        3610         &        3073         &        3073         &        3579         &        3579         \\


==> include_OLD/MoB_ks_23me_ukb.tex <==
            &\multicolumn{2}{c}{Key Stage 1}            &\multicolumn{2}{c}{Key Stage 2}            &\multicolumn{2}{c}{Key Stage 3}            &\multicolumn{2}{c}{Key Stage 4}            \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\midrule
Treated     &       0.635\sym{***}&       0.667\sym{***}&       0.277\sym{***}&       0.217\sym{***}&       0.200\sym{*}  &       0.234\sym{**} &       0.256\sym{***}&       0.272\sym{***}\\
            &     (0.019)         &     (0.052)         &     (0.015)         &     (0.040)         &     (0.079)         &     (0.058)         &     (0.028)         &     (0.031)         \\
\addlinespace
Treated*PGI &                     &      -0.073         &                     &      -0.071\sym{***}&                     &      -0.050\sym{*}  &                     &      -0.041\sym{*}  \\
            &                     &     (0.038)         &                     &     (0.017)         &                     &     (0.022)         &                     &     (0.020)         \\
\addlinespace
Treated*MoB &       0.056\sym{***}&       0.050\sym{**} &       0.084\sym{***}&       0.081\sym{***}&       0.020         &       0.016         &       0.024         &       0.020         \\
            &     (0.013)         &     (0.015)         &     (0.012)         &     (0.011)         &     (0.029)         &     (0.031)         &     (0.014)         &     (0.013)         \\
\addlinespace
MoB*PGI     &                     &       0.040\sym{***}&                     &       0.011         &                     &      -0.013         &                     &       0.019\sym{***}\\
            &                     &     (0.003)         &                     &     (0.013)         &                     &     (0.012)         &                     &     (0.004)         \\
\addlinespace
MoB*PGI*Treated&                     &      -0.012         &                     &       0.015         &                     &       0.046\sym{***}&                     &      -0.002         \\
            &                     &     (0.011)         &                     &     (0.011)         &                     &     (0.011)         &                     &     (0.011)         \\
\addlinespace
MoB         &      -0.091\sym{***}&      -0.085\sym{***}&      -0.098\sym{***}&      -0.098\sym{***}&      -0.025         &      -0.023         &      -0.039\sym{**} &      -0.037\sym{**} \\
            &     (0.013)         &     (0.015)         &     (0.011)         &     (0.008)         &     (0.014)         &     (0.014)         &     (0.011)         &     (0.010)         \\
\addlinespace
PGI         &       0.261\sym{***}&       0.256\sym{***}&       0.346\sym{***}&       0.341\sym{***}&       0.358\sym{***}&       0.341\sym{***}&       0.319\sym{***}&       0.325\sym{***}\\
            &     (0.015)         &     (0.017)         &     (0.010)         &     (0.034)         &     (0.015)         &     (0.037)         &     (0.007)         &     (0.024)         \\
\midrule
R2          &       0.175         &       0.182         &       0.145         &       0.150         &       0.143         &       0.146         &       0.141         &       0.144         \\
Observations&        3436         &        3436         &        3610         &        3610         &        3073         &        3073         &        3579         &        3579         \\


==> include_OLD/MoB_ks_plink.tex <==
            &\multicolumn{2}{c}{Key Stage 1}            &\multicolumn{2}{c}{Key Stage 2}            &\multicolumn{2}{c}{Key Stage 3}            &\multicolumn{2}{c}{Key Stage 4}            \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\midrule
Treated     &       0.590\sym{***}&       0.626\sym{***}&       0.211\sym{***}&       0.159\sym{***}&       0.142         &       0.159\sym{**} &       0.193\sym{***}&       0.223\sym{***}\\
            &     (0.016)         &     (0.052)         &     (0.017)         &     (0.037)         &     (0.081)         &     (0.058)         &     (0.032)         &     (0.034)         \\
\addlinespace
Treated*PGI &                     &      -0.084\sym{**} &                     &      -0.061\sym{*}  &                     &      -0.090\sym{***}&                     &      -0.015         \\
            &                     &     (0.030)         &                     &     (0.026)         &                     &     (0.019)         &                     &     (0.014)         \\
\addlinespace
Treated*MoB &       0.070\sym{***}&       0.068\sym{***}&       0.109\sym{***}&       0.110\sym{***}&       0.044         &       0.048         &       0.048\sym{**} &       0.046\sym{**} \\
            &     (0.011)         &     (0.011)         &     (0.013)         &     (0.012)         &     (0.030)         &     (0.031)         &     (0.015)         &     (0.016)         \\
\addlinespace
MoB*PGI     &                     &       0.013         &                     &       0.007         &                     &       0.033\sym{***}&                     &       0.045\sym{***}\\
            &                     &     (0.006)         &                     &     (0.009)         &                     &     (0.006)         &                     &     (0.009)         \\
\addlinespace
MoB*PGI*Treated&                     &       0.014         &                     &       0.014         &                     &       0.013         &                     &      -0.036\sym{**} \\
            &                     &     (0.009)         &                     &     (0.012)         &                     &     (0.008)         &                     &     (0.010)         \\
\addlinespace
MoB         &      -0.090\sym{***}&      -0.085\sym{***}&      -0.099\sym{***}&      -0.102\sym{***}&      -0.028         &      -0.026         &      -0.042\sym{**} &      -0.042\sym{**} \\
            &     (0.010)         &     (0.011)         &     (0.012)         &     (0.010)         &     (0.015)         &     (0.014)         &     (0.012)         &     (0.012)         \\
\addlinespace
PGI         &       0.237\sym{***}&       0.229\sym{***}&       0.293\sym{***}&       0.301\sym{***}&       0.316\sym{***}&       0.312\sym{***}&       0.276\sym{***}&       0.283\sym{***}\\
            &     (0.010)         &     (0.026)         &     (0.009)         &     (0.015)         &     (0.017)         &     (0.023)         &     (0.012)         &     (0.029)         \\
\midrule
R2          &       0.162         &       0.167         &       0.111         &       0.114         &       0.116         &       0.119         &       0.115         &       0.120         \\
Observations&        3436         &        3436         &        3610         &        3610         &        3073         &        3073         &        3579         &        3579         \\


==> include_OLD/MoB_ks_ukb.tex <==
            &\multicolumn{2}{c}{Key Stage 1}            &\multicolumn{2}{c}{Key Stage 2}            &\multicolumn{2}{c}{Key Stage 3}            &\multicolumn{2}{c}{Key Stage 4}            \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\midrule
Treated     &       0.619\sym{***}&       0.658\sym{***}&       0.249\sym{***}&       0.189\sym{***}&       0.177\sym{*}  &       0.211\sym{**} &       0.232\sym{***}&       0.257\sym{***}\\
            &     (0.018)         &     (0.056)         &     (0.012)         &     (0.040)         &     (0.078)         &     (0.054)         &     (0.026)         &     (0.033)         \\
\addlinespace
Treated*PGI &                     &       0.007         &                     &      -0.023         &                     &      -0.034         &                     &       0.014         \\
            &                     &     (0.036)         &                     &     (0.047)         &                     &     (0.071)         &                     &     (0.013)         \\
\addlinespace
Treated*MoB &       0.067\sym{***}&       0.061\sym{***}&       0.101\sym{***}&       0.102\sym{***}&       0.033         &       0.034         &       0.038\sym{**} &       0.037\sym{**} \\
            &     (0.012)         &     (0.013)         &     (0.012)         &     (0.010)         &     (0.029)         &     (0.033)         &     (0.013)         &     (0.011)         \\
\addlinespace
MoB*PGI     &                     &       0.043\sym{***}&                     &       0.028         &                     &      -0.012         &                     &       0.025\sym{***}\\
            &                     &     (0.006)         &                     &     (0.015)         &                     &     (0.014)         &                     &     (0.003)         \\
\addlinespace
MoB*PGI*Treated&                     &      -0.037\sym{**} &                     &      -0.015         &                     &       0.038         &                     &      -0.027\sym{**} \\
            &                     &     (0.012)         &                     &     (0.019)         &                     &     (0.021)         &                     &     (0.007)         \\
\addlinespace
MoB         &      -0.097\sym{***}&      -0.091\sym{***}&      -0.107\sym{***}&      -0.107\sym{***}&      -0.031\sym{*}  &      -0.030\sym{*}  &      -0.046\sym{***}&      -0.046\sym{***}\\
            &     (0.012)         &     (0.013)         &     (0.010)         &     (0.009)         &     (0.013)         &     (0.014)         &     (0.011)         &     (0.011)         \\
\addlinespace
PGI         &       0.257\sym{***}&       0.232\sym{***}&       0.320\sym{***}&       0.308\sym{***}&       0.331\sym{***}&       0.315\sym{***}&       0.293\sym{***}&       0.291\sym{***}\\
            &     (0.015)         &     (0.021)         &     (0.013)         &     (0.038)         &     (0.016)         &     (0.053)         &     (0.007)         &     (0.023)         \\
\midrule
R2          &       0.173         &       0.183         &       0.129         &       0.136         &       0.126         &       0.130         &       0.126         &       0.129         \\
Observations&        3436         &        3436         &        3610         &        3610         &        3073         &        3073         &        3579         &        3579         \\


==> include_OLD/sumstats.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{ccccc}}
\toprule
                    &\multicolumn{5}{c}{}                                            \\
                    &        mean&         p50&         min&         max&          sd\\
\midrule
Home score          &    8.147453&           8&           0&          12&    2.205964\\
Mother's parenting score&    10.49545&          11&           0&          12&    1.495952\\
Partner's parenting score&    23.54768&          24&          10&          30&    3.781217\\
Teaching score carer&    8.008982&           8&           0&          11&    2.174171\\
Teaching score carer&    6.576195&           7&           0&           8&    1.206814\\
Teaching score      &    6.936799&           7&           0&           8&    1.147933\\
FREQ MUM Talks to CH During Housework&    4.543179&           5&           1&           5&    .6451142\\
Freq.carer talks to child when occupied&     4.49805&           5&           1&           5&     .648378\\
Times MUM Talks to CH when Occupied&    4.402184&           5&           1&           5&    .6931504\\
FREQ CH Taken to Library&    4.147734&           5&           1&           5&    1.020923\\
Frequency child goes to library&    3.950204&           4&           1&           5&    1.045937\\
FREQ CH Taken to Library&    3.709295&           4&           1&           5&    1.035221\\
FREQ CH Taken to Places of Interest&    3.392375&           4&           1&           5&    .8553522\\
Frequency child visits place of interest&    3.299828&           3&           1&           5&     .798385\\
FREQ CH Taken to Places of Interest&    3.325798&           3&           1&           5&    .7721977\\
No of books child has&    3.877874&           4&           1&           4&    .3655757\\
NO of Books CH Owns &    3.946745&           4&           1&           4&    .2441194\\
\midrule
Observations        &        7310&            &            &            &            \\
\bottomrule
\end{tabular}
}

